SelfVoxeLO: Self-supervised LiDAR Odometry with Voxel-based Deep Neural Networks

Recent learning-based LiDAR odometry methods have demonstrated their competitiveness. However, most methods still face two substantial challenges: 1) the 2D projection representation of LiDAR data cannot effectively encode 3D structures from the point clouds; 2) the needs for a large amount of labeled data for training limit the application scope of these methods. In this paper, we propose a self-supervised LiDAR odometry method, dubbed SelfVoxeLO, to tackle these two difficulties. Specifically, we propose a 3D convolution network to process the raw LiDAR data directly, which extracts features that better encode the 3D geometric patterns. To suit our network to self-supervised learning, we design several novel loss functions that utilize the inherent properties of LiDAR point clouds. Moreover, an uncertainty-aware mechanism is incorporated in the loss functions to alleviate the interference of moving objects/noises. We evaluate our method's performances on two large-scale datasets, i.e., KITTI and Apollo-SouthBay. Our method outperforms state-of-the-art unsupervised methods by 27%/32% in terms of translational/rotational errors on the KITTI dataset and also performs well on the Apollo-SouthBay dataset. By including more unlabelled training data, our method can further improve performance comparable to the supervised methods.

==> figure/network_details.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=1\linewidth, trim=0cm 10cm 1cm 0cm, clip]{figure/_network_details.pdf}
    \caption{The design details of our proposed modules.}
    \label{fig:framework}
    % \vspace{-4ex}
\end{figure*}

==> figure/traj_plot_sup.tex <==
\begin{figure}
    \centering
% \resizebox{0.6\linewidth}{!}{
    \begin{subfigure}[t]{0.7\textwidth}
        \includegraphics[width=\linewidth, trim=1.9cm 12.5cm 19cm 0cm, clip]{figure/traj_plot2.pdf}
    % \caption{}
    \end{subfigure}
    \caption{Trajectory plots comparison among some two-frame methods on KITTI. }\label{fig:traj_plot}
\vspace{-3ex}
\end{figure}


==> table/runtime_compare.tex <==
\begin{minipage}{\textwidth}
  \centering 

  \vskip\baselineskip
  \begin{minipage}[]{\textwidth}
    \centering
    \parbox{1\linewidth}{
      \centering
    \captionof{table}{The runtime comparison among different methods.}\label{tab:runtime_comparison}
    \resizebox{0.3\linewidth}{!}{
      \begin{tabular}{c|*{2}{c}}
        \hline
        Methods & Time (ms) \\
        \hline 
        ICP-po2po~\cite{arun1987least} & 261\\
        ICP-po2pl~\cite{chen1992object} & 1250\\
        GICP~\cite{segal2009generalized} & 1781\\
        NDT-P2D~\cite{stoyanov2012fast} & 1723\\
        CLS~\cite{velas2016collar}& 19843 \\
        % LOAM & \\
        Ours&88.4 \\
        \hline
      \end{tabular}
    }
    }
    \end{minipage}
  \end{minipage}


